Nexus Machine: An Active Message Inspired Reconfigurable Architecture for Irregular Workloads

Modern reconfigurable architectures are increasingly favored for resource-constrained edge devices as they balance high performance, energy efficiency, and programmability well. However, their proficiency in handling regular compute patterns constrains their effectiveness in executing irregular workloads, such as sparse linear algebra and graph analytics with unpredictable access patterns and control flow. To address this limitation, we introduce the Nexus Machine, a novel reconfigurable architecture consisting of a PE array designed to efficiently handle irregularity by distributing sparse tensors across the fabric and employing active messages that morph instructions based on dynamic control flow. As the inherent irregularity in workloads can lead to high load imbalance among different Processing Elements (PEs), Nexus Machine deploys and executes instructions en-route on idle PEs at run-time. Thus, unlike traditional reconfigurable architectures with only static instructions within each PE, Nexus Machine brings dynamic control to the idle compute units, mitigating load imbalance and enhancing overall performance. Our experiments demonstrate that Nexus Machine achieves 90% better performance compared to state-of-the-art (SOTA) reconfigurable architectures, within the same power budget and area. Nexus Machine also achieves 70% higher fabric utilization, in contrast to SOTA architectures.

==> Backup_ISCA/evaluation_backup.tex <==
\section{Experimental Evaluations}

\subsection{Baseline Architectures}
We evaluate \textit{Nexus Machine} against two baseline architectures, \textit{Generic CGRA} and \textit{TIA-like} modeled after HyCube~\cite{hycube} and Triggered Instructions~\cite{tia}, respectively, with the following architectural parameters for fair evaluations.

\textbf{PE array:} The PE array consists of 16 PEs interconnected with a mesh NoC where each router hop takes a cycle.
\textit{TIA-like} and \textit{Nexus Machine} have a dynamic NoC with 16 identical PEs.
In contrast, \textit{generic CGRA} has a static NoC, controlled by router configurations, with 4 memory PEs positioned at a boundary column and 12 regular PEs. 
%\textcolor{red}{explain why TIA needs dynamic NoC while HyCUBE can use static NoC. Myabe draw a figure to show the 3 architectures if you have space?}
\begin{comment}
{\color{blue} \textbf{Data memory:} \textit{TIA-like} and \textit{Nexus Machine} have 16KBx16 dual port memories, locally connected to each PE.
Whereas, \textit{generic CGRA} has 64KBx4 single-port memories accessible by the boundary PEs.}
\end{comment}

\textbf{Data memory:}  \textit{TIA-like} architecture incorporates 16KBx16 dual-port memories, while the \textit{Nexus Machine} has 8KBx16 dual-port memories and 8KBx16 \textit{AM Queues} per PE. Whereas, \textit{generic CGRA} has 64KBx4 dual-port memories accessible only by boundary PEs.

\textbf{Configuration memory:} \textit{TIA-like} and \textit{Nexus Machine} have 8 entries of 10 bits each to fit the selected benchmarks.
\textit{Generic CGRA} has 8 entries of 64 bits to fit the ALU and router configurations. As \textit{TIA-like} and \textit{Nexus Machine} use dynamic NoC, router configurations are not required, so each entry is 10 bits long.
%All the three architectures are evaluated with 16 PEs, and 
%Table~\ref{table:arch_parameters} shows the architectural parameters used for evaluations.

\subsection{Benchmarks}
\begin{table}[h!]
    \centering
    \resizebox{0.85\columnwidth}{!} {
    \begin{tabular}{rrrr} \hline \rule{0pt}{2.5ex} 
    \textbf{Kernel}&  \textbf{Name}&  \textbf{Dimensions}& \textbf{Density (in \%)}\\ \hline
    %[1mm]
    %& & &\textbf{(in \%)}\\[1mm]
    %\hline \rule{0pt}{2.5ex} 
    
        
    %New Entry%      
    SpMV &  Resnet50 \#50~\cite{resnet50}&  
& \\[1mm]
 & Weights& $2048 \bullet 1000 $&13.03\\ \hline \rule{0pt}{2.5ex}  
    
    %New Entry%      
    SpMSpM &  Resnet50 \#40&  & \\
 & Weights& $512 \bullet 1024$&39.05\\ 
    & Input Activations& $1024 \bullet 196$&46.04
        \\[1mm]\hline \rule{0pt}{2.5ex} 

 %    %New Entry% 
 %    Conv &  Resnet50 \#13&  & \\[1mm]
 % & Weights& $28 \bullet 3 \bullet 128 \bullet 128$&42.50\\\hline \rule{0pt}{2.5ex}   

    %New Entry% 
    SDDMM &  DEiT-Base \#1~\cite{deit}&  & 
            \\
 & Mask& $197 \bullet 197$&\\  
    & Score& $197 \bullet 64$&9.82
        \\[1mm] \hline \rule{0pt}{2.5ex}   

    %New Entry% 
    SpM+SpM &  Resnet50 \#3&  & \\[1mm]
 & 64 Convoluted& $64 \bullet56 \bullet 56$&40.77 \\
 & Matrices & &(average)\\\hline
 Sparse& Resnet50 \#40& &\\
 Convolution& Weights& $3 \bullet 3$&\\
 & Input Activations& $1024 \bullet 196$&46.04\\\hline
 MatMul& Resnet50 \#40& &        \\
 & Weights& $512 \bullet 1024$&100\\
 & Input Activations& $1024 \bullet 196$&100\\\hline
 Dense& Resnet50 \#40& &\\
  Convolution& Weights& $3 \bullet 3$ &100\\
 & Input Activations& $1024 \bullet 196$&100\\\hline  BFS, SSSP&  infect-dublin~\cite{idublin} &  & \\
     %New Entry% & Nodes& 410&3.03\\
 & Nodes& 410&3.03\\[1mm]\hline
    
    \end{tabular}
  }
    \caption{Datasets used for evaluating \textit{Nexus Machine}}
    \label{table:datasets}
\end{table}
%\textcolor{red}{this is a good place to explain what classes of applications you can handle. Is it sparse tensors only? Then SSSP is using incidence matrix? Should also be included in introduction}
\begin{comment}
\textit{Nexus Machine} is designed for accelerating irregular workloads including sparse tensor algebra and graph analytics, specifically for performing computations on sparse tensors.
We evaluated \textit{Nexus Machine} on six workloads, as illustrated in Table~\ref{table:datasets}.
%We evaluated \textit{Nexus Machine} on six Irregular workloads from sparse tensor algebra and graph analytics, as illustrated in Table~\ref{table:datasets}.\\

\textbf{Sparse Matrix-Vector Multiplication (SpMv)} multiplies a Sparse Matrix in CSR format with a Dense Vector. 
\textbf{Sparse Matrix Multiplication (SpMSpM)} multiplies two Sparse matrices, both in CSR format. Our baselines are based on Gustavson's algorithm (Row-based) as it is an asymptotically efficient parallel algorithm that processes one output row at a time. It is an important linear algebra benchmark and manifests in many applications at the edge, including Pruned CNNs and Sparse Attention~\cite{sanger, vitcod}.
%\textbf{Convolution (Conv)} takes one sparse matrix in CSR format and convolves it with a dense kernel. For our baselines, we evaluate the output-stationary model.
\textbf{Sparse Matrix Addition (M+M)} involves summing two matrices in CSR format element-wise. 
%For our baselines, we consider the binary mask of the output to be precomputed and used as the tensor for AM generation. 
%We consider the binary mask of the output to be precomputed, which serves as the tensor for AM generation.
It is an important benchmark as CNNs accumulate intermediate feature maps across the output channels to get the final output activation.
%\textbf{Sampled Dense-Dense Matrix Multiplication (SDDMM)} is a crucial kernel that finds applications in various settings, including Sparse Attention and Graph Neural Networks. This operation computes the product of two dense matrices by evaluating them only at the non-zero entries of a sparse matrix in CSR format. The sparse matrix serves as the tensor for AM generation.
\textbf{Sampled Dense-Dense Matrix Multiplication (SDDMM)} is a crucial kernel used in Sparse Attention and Graph Neural Networks. It computes the product of two dense matrices by evaluating them only at the non-zero entries of a sparse matrix in CSR format, which serves as the tensor for AM generation.

In graph analytics, \textbf{Breadth-First Search (BFS)} is a fundamental graph traversal algorithm to determine the vertices at a specific distance from the source node.
\textbf{Single shortest path (SSSP)} is the problem of finding a path between two vertices in a graph such that the sum of the weights of its constituent edges is minimized.
For our experiments, we represent graphs using adjacency matrices.
\end{comment}
\textit{Nexus Machine} is designed to accelerate irregular workloads, such as sparse tensor algebra and graph analytics. We evaluated \textit{Nexus Machine} on sparse, dense, and graph workloads to demonstrate its generality; details on the benchmarks are provided in Table~\ref{table:datasets}.

\textbf{Sparse Matrix-Vector Multiplication (SpMv)} involves multiplying a sparse matrix in CSR format with a dense vector. \textbf{Sparse Matrix Multiplication (SpMSpM)} multiplies two sparse matrices, both in CSR format, using Gustavson's algorithm (row-wise), a key benchmark in edge applications including Pruned CNNs and Sparse Attention~\cite{sanger, vitcod}. \textbf{Sparse Matrix Addition (M+M)} sums two sparse matrices in CSR format element-wise, an important benchmark as CNNs accumulate intermediate feature maps across the output channels to get the final output activation.
\textbf{Sampled Dense-Dense Matrix Multiplication (SDDMM)} computes the product of two dense matrices by evaluating them only at the non-zero entries of a sparse matrix in CSR format, relevant for Sparse Attention and Graph Neural Networks.
\textbf{Sparse Convolution} involves convolving a sparse kernel with sparse activations, crucial for CNN workloads where both weights and activations are pruned~\cite{activation_sparsity}.
\textbf{Dense Matrix Multiplication} multiplies two dense matrices, a critical workload for CNNs and LLMs, while \textbf{Dense Convolution} involves a dense kernel with dense activations, essential for CNNs.

In graph analytics, \textbf{Breadth-First Search (BFS)} explores vertices at a specified distance, \textbf{Single Source Shortest Path (SSSP)} finds minimum-weight paths, and \textbf{PageRank} ranks nodes based on connectivity, useful in search engines and social networks. Graphs are represented with adjacency lists in our experiments.
%In graph analytics, \textbf{Breadth-First Search (BFS)} is used to traverse and identify vertices at a specific distance from the source node, while \textbf{Single Shortest Path (SSSP)} finds the minimum weight path between two vertices. {\textbf{PageRank} is an algorithm that ranks nodes in a graph based on their connectivity and importance, commonly used in web search engines, social network analysis, and recommendation systems. \color{blue} Graphs are represented using adjacency list for our experiments.}
\begin{comment}
\textit{Nexus Machine} is designed to accelerate irregular workloads, such as sparse tensor algebra and graph analytics. We evaluated it on sparse, dense, and graph workloads to demonstrate its generality; benchmark details are provided in Table~\ref{table:datasets}.

\textbf{Dense Matrix Multiplication} multiplies two dense matrices, a critical workload for CNNs and LLMs, while \textbf{Dense Convolution} involves a dense kernel with dense activations, essential for CNNs. \textbf{Sparse Matrix-Vector Multiplication (SpMV)} multiplies a sparse matrix in CSR format with a dense vector, and \textbf{Sparse Matrix Multiplication (SpMSpM)} multiplies two sparse matrices using Gustavson’s row-wise algorithm, important for Pruned CNNs and Sparse Attention~\cite{sanger, vitcod}. \textbf{Sparse Matrix Addition (M+M)} sums two sparse matrices element-wise in CSR format, a key benchmark for accumulating CNN feature maps across output channels. \textbf{Sampled Dense-Dense Matrix Multiplication (SDDMM)} multiplies two dense matrices, evaluated only at non-zero entries of a sparse matrix, relevant to Sparse Attention and Graph Neural Networks. \textbf{Sparse Convolution} involves convolving sparse kernels with sparse activations, crucial for pruned CNN workloads~\cite{??}.

In graph analytics, \textbf{Breadth-First Search (BFS)} explores vertices at a specified distance, \textbf{Single Source Shortest Path (SSSP)} finds minimum-weight paths, and \textbf{PageRank} ranks nodes based on connectivity, useful in search engines and social networks. Graphs are represented with adjacency lists in our experiments.
\end{comment}
\vspace{-0.4cm}
\subsection{Experimental Setup}
We evaluate \textit{Nexus Machine}'s and \textit{TIA-like} architecture's performance using a custom-written cycle-accurate simulator that models dynamic routers, congestion control, and backpressure signaling. 
Benchmarks are mapped to \textit{configuration memory} and \textit{AM Queues} for simulation with datasets specified in Table~\ref{table:datasets}.
For SpMv, SpMSpM, and SpM+SpM, we use a ResNet-50~\cite{resnet50} model, pruned and fine-tuned to maintain accuracy. SpMSpM involves transforming convolution layers into matrices via Toeplitz~\cite{toeplitz}. SDDMM is evaluated with a sparse input mask similar to ViTCoD~\cite{vitcod}, and graph datasets are partitioned using Metis~\cite{metis} for load balancing.
%We simulate the \textit{generic CGRA} with LLVM-based Morpher~\cite{morpher} mapping and model bank conflicts during irregular workloads. 
We simulate the \textit{generic CGRA} using the mapping information provided by the LLVM-based Morpher~\cite{morpher} tool and model bank conflicts during irregular workloads. 

All architectures are modeled in System Verilog HDL, synthesized on a commercial 22 nm FDSOI process using Cadence Genus at 100MHz. The foundry’s memory-compiled SRAM cells are used to model the memories.
\textit{Nexus Machine} is synthesizable with a maximum clock frequency of 588MHz.
We verify functionality through behavioral simulations at the RTL level, using test inputs to generate VCD files and calculate an average toggle rate of 0.12 to 0.2 for the compute logic. For conservative power estimates, we apply a higher default toggle rate of 0.25 in Cadence Genus for post-synthesis netlist estimations.
\subsection{Experimental Results}
\begin{figure}[h!]
	\scriptsize
	\centering
	\input{graphs/performance}
	\caption{Performance of \textit{generic CGRA} and \textit{TIA-like} architectures across workloads (in cycles), normalized to \textit{Nexus Machine}.} 
	\label{fig:performance}
	%\vspace{-.5cm}
\end{figure}
%\textcolor{red}{\bf Peh: Is your legend in Fig 10 wrong?}
\vspace{-0.8cm}
\begin{figure}[h!]
	\scriptsize
	\centering
	\input{graphs/innetworkcomp}
	\caption{\textit{Nexus Machine}: Percentage of total computations performed in-network.} 
	\label{fig:innetworkcomp}
	%\vspace{-.5cm}
\end{figure}
\vspace{-0.8cm}
\begin{figure}[h!]
	\scriptsize
	\centering
	\input{graphs/utilization}
	\caption{Total Fabric Utilization} 
	\label{fig:utilization}
	%\vspace{-.5cm}
\end{figure}
\vspace{-0.5cm}
\begin{figure}[h!]
	\scriptsize
	\centering
    \input{graphs/congestion}
	%\includegraphics[width=0.9\columnwidth]{content/graphs/congestion1.png}
	\caption{Total Network Congestion} 
	\label{fig:congestion}
\end{figure}
\vspace{-0.2cm}
\begin{figure}[h!]
	\scriptsize
	\centering
	\input{graphs/network_traffic}
	\caption{Network Traffic Overhead: Extra data transmitted over NoC in \textit{Nexus Machine} relative to \textit{TIA-like} architecture.}
	\label{fig:network_overhead}
	%\vspace{-.5cm}
\end{figure}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

{\bf Overall Performance.}
We assess the performance of each benchmark by monitoring the number of cycles required for execution completion on each of the architectures. Fig.~\ref{fig:performance} presents number of cycles normalized to that of \textit{Nexus Machine}.
\textit{Nexus Machine} outperforms \textit{generic CGRA} and \textit{TIA-like} baselines by an average of 1.7x and 1.5x respectively. For SDDMM, \textit{Nexus Machine} outperforms \textit{generic CGRA} and \textit{TIA-like} by 2.07x and 1.88x, respectively.

We also analyze the distribution of cycles spent by the fabric for 1) useful computations and 2) idle cycles. 
%As anticipated, indirect memory accesses and stalls consume a significant portion of cycles in both \textit{Conventional} and \textit{Dataflow} baselines. However, \textit{Nexus Machine} effectively addresses this issue by bringing compute to these idle ALUs.
\textit{Nexus Machine} performs better for all the benchmarks in comparison to both the baselines.
As anticipated, both \textit{generic CGRA} and \textit{TIA-like} baselines have substantial overheads due to stalls attributed to bank conflicts and load imbalance, respectively. 
However, \textit{Nexus Machine} effectively mitigates this issue by dynamically bringing compute to the idle ALUs, thus reducing the number of stalls significantly. 
%\textcolor{red}{state first which benchmarks Nexus does better. Also explain where TIA does better or worse than generic and why}

For the SpMv and SpM+SpM workloads, \textit{generic CGRA} outperforms the \textit{TIA-like} baseline due to a lower number of unroll factor, effectively mitigating bank conflicts during execution. Thus, leading to a superior performance for these workloads.
Additionally, the SpM+SpM workload has denser tensor computations, further favoring the performance of the \textit{generic CGRA}.
%\textcolor{blue} {\bf Peh: Explain why TIA-like does worse than generic CGRA for SpMV and SpM+SpM -- poor control placement vs. compiler-driven placement of CGRA?} 
%For SDDMM, \textit{Nexus Machine} outperforms both the baselines significantly.
%This is because of low network congestion in the case of \textit{Nexus Machine}.
For SDDMM, \textit{Nexus Machine} performs significantly better compared to both the baselines.
This is primarily attributed to the reduced network congestion observed in the case of \textit{Nexus Machine}.
%{\bf Peh: Explain why TIA doesn't do well for SDDMM while Nexus does with some submetrics, cos in-network computation percentage is only 20\%, not high either, so more insight needed}
However, for dense workloads, \textit{TIA-like} outperforms \textit{Nexus Machine}, as opportunistic execution increases network congestion.
On average, \textit{Nexus Machine} requires 40\% and 32\% fewer cycles than \textit{generic CGRA} and \textit{TIA-like} baselines, respectively.

{\bf In-network computations.}
For \textit{Nexus Machine}, Fig.~\ref{fig:innetworkcomp} shows the percentage of in-network computations performed during routing of active messages.
\textit{Nexus Machine} performs 41.8\% of computations in-network on average, addressing load balancing in irregular workloads and improving fabric utilization.
For dense workloads, this drops to 2–3\% as all PEs are fully utilized.
%\textcolor{red}{explain the variation across benchmarks}

%Static pipeline CGRAs take higher number of cycles in all kernels, primarily due to their limitations in handling imbalanced branches. In such scenarios, the additional operations in the longer execution path cannot be effectively merged into the shorter ones, leading to increased cycle counts.

{\bf Fabric Utilization.} 
%\textcolor{red}{Why TIA utilization is worse than generic?}
Fabric Utilization denotes the percentage of PE fabric effectively performing computations during the entire execution.
Fig.~\ref{fig:utilization} illustrates the percentage of fabric utilization for each benchmark. \textit{Nexus Machine} exhibits consistently higher utilization than all the baselines. This can be primarily attributed to the \textit{AM Network Interface} logic, which reduces irregular memory loads, and in-network computations employed by \textit{Nexus Machine}'s architecture.

{\bf Network Congestion.}
Fig.~\ref{fig:congestion} presents the breakdown of network congestion in the fabric across all the input ports. \textit{Nexus Machine} mitigates the average network congestion by 13\%, compared to the \textit{TIA-like} baseline. It notably reduces congestion at the LOCAL port, which has the most substantial impact on overall runtime.
The routing congestion for \textit{generic CGRA} baseline is omitted, as it employs static routing that is determined at compilation time.
Compilation time for \textit{generic CGRA} averages around 7.22 sec due to its extensive static route search, as compared to just 0.55 sec for \textit{Nexus Machine} that performs hardware-based routing supported by AMs.

{\bf Area and Power.}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t!]
    \resizebox{\columnwidth}{!} {
    \centering
    \begin{tabular}{cccc} \hline 
        \textbf{Component}&  \textbf{Sub module}&  \textbf{Area (in mm$^2$)} & \textbf{Power (in mW)}\\ \hline 
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Memory\end{tabular}}&  AM Queue&  0.0350& 0.4938\\ \cline{2-4}  
        & Config Memory& 0.0144&0.1611\\ \cline{2-4} 
        &  Data Memory&  0.0243& 0.5621\\ \hline
        Compute Unit& ALU& 0.0004&0.4419\\ \hline 
         \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Interconnect\end{tabular}}&  Logic&  0.0255& 2.0014\\ \cline{2-4}
        & Buffers& 0.0044&0.1406\\ \hline
        Scanners&  &  0.0023& 0.0728\\ \hline
        Extra& & 0.0078&0.065\\ \hline 
        Total&  &  0.1138& 3.938\\ \hline
    \end{tabular}
    }
    \caption{\textit{Nexus Machine}: Area and Power breakdown} 
    \label{table:synth_results}
\end{table}
%\vspace{2mm}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lcc}
\hline
\textbf{Architecture}                          & \textbf{Area (in mm$^2$)}& \textbf{Power (in mW)}\\ \hline
Generic CGRA&                     0.1035&                     2.961\\ \hline
TIA-like&                     0.1122&                     4.626\\ \hline
Nexus Machine&                     0.1138&                     3.938\\\hline
\end{tabular}%
}
\caption{Total Area and Power Comparisons for different architectures}
\label{table:synth_results_comparison}
\end{table}
Table~\ref{table:synth_results} presents a detailed breakdown of the area and power consumption for \textit{Nexus Machine}. 
\textit{Crossbar}, \textit{AM queues} and \textit{data memories} consume a significant portion of both area and power, while bit-vector scanners account for negligible area and power consumption.
%\textcolor{red}{\bf Peh: Scanners are considered extra? Their area/power overhead was not mentioned earlier and shd be briefly noted here.}

Table~\ref{table:synth_results_comparison} compares total area and power across the three architectures.
\textit{Nexus Machine} shows a slight area increase over the \textit{generic CGRA} due to the inclusion of \textit{AM Queues} and dynamic router buffers.
Its router logic consumes more power, primarily due to the crossbar handling more bits than \textit{generic CGRAs} and \textit{TIA-like}.
\textit{Generic CGRA} has larger configuration memory to store both ALU and router configurations.
\textit{TIA-like} has minor area and power overhead compared to \textit{Nexus Machine} from added tag-matching and scheduler logic.
\begin{comment}
\subsubsection{Power}
The power consumption is obtained from synthesis, as mentioned above. The power distribution of all the architectures is outlined in Table~\ref{table:synth_results}.
\iffalse Notably, the AM Generation logic contributes significantly to the overall power consumption of Nexus Machine due to the presence of FIFOs.\fi
\end{comment}

{\bf Power Efficiency.}
Table~\ref{tab:power_efficiency} shows the effective power efficiency. \textit{Nexus Machine} achieves a better average and peak power efficiency than the baselines.
\textit{Nexus Machine} achieves an average power efficiency of 139MOPS/mW across all the benchmarks, and a peak power efficiency of 191MOPS/mW.

{\bf Area Efficiency.}
Table~\ref{tab:power_efficiency} compares the area efficiency of \textit{Nexus Machine} with the baselines. 
\textit{Nexus Machine} demonstrates higher average area efficiency, achieving 4.7GOPS/mm$^2$.

We can conclude that \textit{Nexus Machine} provides a better trade-off between power, area and performance, achieving the highest power and area efficiency among the compared architectures.

{\bf Network Traffic.}
\iffalse
Network traffic refers to the data transferred during the execution of workloads.
Figure~\ref{fig:network_overhead} illustrates the network traffic overhead of Nexus Machine in comparison to TIA-like architecture.
Nexus Machine experiences an average of 13.89\% additional network traffic overhead. Note that this is due to the wider NoC of Nexus, to accommodate the additional information needed to encode AMs; There is no extra network packets in Nexus, nor any additional network latency or unnecessary hop count, as AMs are launched along the way to the destination with Nexus Machine's lazy execution. In other words, Nexus incurs higher NoC area overhead, instead of performance overhead.
\fi
Network traffic refers to the data transferred over NoC during execution of workloads.
Fig.~\ref{fig:network_overhead} compares the network traffic overhead of \textit{Nexus Machine} with a \textit{TIA-like} architecture.
\textit{Nexus Machine} exhibits an average of 26.32\% additional network traffic overhead.
This is due to the \textit{Nexus Machine}'s wider NoC required to accommodate the extra information for encoding AMs.
It's important to note that \textit{Nexus Machine} doesn't introduce extra network packets, latency, or additional hops. 
This is because AMs are efficiently launched along the route to their destination using the opportunistic execution approach. 
Essentially, \textit{Nexus Machine} incurs higher NoC area overhead instead of performance overhead.

%\textcolor{red}{Peh: Quantify how much higher area overhead. Explain why there is NoC area overhead? Cos actually, Nexus' has a narrower NoC, and the dynamic NoC has simple logic. Is it due to the AM queues being counted as part of NoC? If so, explain}


\begin{table}
    \centering
    \resizebox{0.95\columnwidth}{!} {
    \begin{tabular}{cccc} \hline 
         \textbf{Architecture} &   \textbf{Average Power}&\textbf{Peak Power} &\textbf{Average Area}\\
         &  \textbf{Efficiency}&\textbf{Efficiency} &\textbf{Efficiency}\\
 & \textbf{(in MOPS/mW)}&\textbf{(in MOPS/mW)} & \textbf{(in GOPS/mm$^2$)}\\ \hline
         Generic CGRA*&   110&123 &3.1\\ \hline 
         TIA-like*&   72&106 &2.9\\ \hline
 Nexus Machine& 137&191&4.7\\\hline
    \end{tabular}
    }
    %\vspace{-.2cm}
    \begin{flushleft}
    \tiny{*These numbers are specific to the evaluated irregular workloads and may differ from those reported in other works.}
    \end{flushleft}
    %\vspace{-.1cm}
    \caption{Power and Area Efficiency Comparisons for different architectures}
    \label{tab:power_efficiency}
\end{table}

%{\color{blue}\subsection{Scalability}
%}

\subsection{Discussion: Generality at the expense of configuration memory}
For the \textit{Nexus Machine}, the flexibility and generality come at the cost of storing all instructions within every PE.
While most of the irregular kernels evaluated typically require only a few configurations, this can be challenging for bigger workloads. 
One optimization for bigger workloads is to limit half of the instructions to alternate PEs and the remaining instructions to the others.
This approach restricts PE flexibility but improves configuration memory efficiency.
We evaluated this approach using \textit{PageRank}, where \textit{Nexus Machine} showed superior performance by achieving 48\% fabric utilization, compared to 15\% for \textit{generic CGRAs} and 40\% for \textit{TIA-like}.






Fig.~\ref{fig:edp} presents Energy-Delay product comparison of all evaluated architectures. While \textit{Nexus Machine} incurs slight overhead versus dense-specialized designs, this is offset by the diversity of modern AI workloads. These include sparsity in both weights and activations in models like ResNet-50, and operator combinations such as SDDMM and SpMSpM in language models like Llama-8B and Mistral-7B. \textbf{This variability underscores the need for architectures like \textit{Nexus Machine} that adapt to data sparsity through dynamic reconfigurable execution.}

==> content/compiler_backup.tex <==
\vspace{-0.365cm}
\subsection{Programming Nexus Machine}
\begin{comment}
The program is provided as a C-based code that indicates the loop iterations.
The programmer is responsible for explicitly annotating independent loop iterations. 
Similar to previous parallel programming paradigms (e.g., OpenMP, CUDA), the programmer annotates outer loops containing independent loop nests using the \textit{parallel-for} keyword.
\textit{Nexus Machine} proceeds to compile and execute the program, with each iteration of the \textit{parallel-for} loop executed independently but with sequential semantics. 
A loop with dependencies that is incorrectly marked \textit{parallel-for} will execute with undefined semantics.
\end{comment}
\begin{comment}
The program is written in C code that specifies loop iterations. 
The programmer must explicitly annotate independent loop iterations. 
Similar to other parallel programming paradigms (e.g., OpenMP, CUDA), the programmer uses the \textit{parallel-for} keyword to annotate outer loops with independent loop nests. 
\textit{Nexus Machine} then compiles and executes the program, with each \textit{parallel-for} loop iteration running independently but maintaining sequential semantics. 
If a loop with dependencies is incorrectly marked as \textit{parallel-for}, it will execute with undefined behavior.
\end{comment}
\begin{comment} The program is written in C with loop iterations specified by the programmer. Independent loop iterations must be explicitly annotated using the \textit{parallel-for} keyword, similar to OpenMP or CUDA. \textit{Nexus Machine} compiles and executes the program, running each \textit{parallel-for} loop iteration independently while preserving sequential semantics. Incorrectly annotating dependent loops as \textit{parallel-for} will result in undefined behavior.\end{comment}
{Nexus targets affine loops with associative operations, using the polyhedral model to enable parallel execution, especially for AI workloads involving reduction loops. Programs are written in C, where the programmer annotates independent loop iterations with \textit{parallel-for} keyword, similar to OpenMP or CUDA. The compiler supports nested loops and fully unrolls annotated loops, maximizing parallelism across all levels. Each iteration is flattened, ensuring sequential execution of instructions within each iteration to maintain intra-iteration dependencies. It is the programmer’s responsibility to ensure correct annotations for non-assocaiative inter-iteration dependencies. \textit{Nexus Machine} compiles and executes the program, running each \textit{parallel-for} loop iteration independently while preserving sequential semantics. Incorrectly annotating dependent loops as \textit{parallel-for} will result in undefined behavior. An example SpMV code illustrating these annotations is provided in Fig. 5.
%Any incorrectly marked dependencies within loops are flagged as errors by the \textit{Nexus Machine}'s static compiler {\color{blue} using the \textit{Loop Vectorizer} pass in LLVM}.
\vspace{-0.39cm}
\subsection{Nexus Machine Compiler}
\label{section:compiler}
\begin{figure}[h!]
	\scriptsize
	\centering
	\includegraphics[width=\columnwidth]{diagrams/compiler.pdf}
	\caption{Process for transforming an application code and data into configuration and data format for \textit{Nexus Machine}.}
	\label{fig:compiler}
	%\vspace{-.5cm}
\end{figure}

\begin{comment}
\begin{algorithm}[!t]
\small
\caption{DFG generation}
\label{alg:labelAwareSA}
Identify backedges and connect basic blocks \;
Get transfer variables among nested loops \;
Convert LLVM IR instruction into DFG nodes \;
Set data dependency constraints \;
Remove redundant and dead DFG nodes \;
Sort DFG nodes by ASAP order \;
\KwIn{Source code, annotated loop;}
\KwOut{DFG}
\end{algorithm}
\end{comment}

\textit{Nexus Machine} integrates a static compiler responsible for preprocessing the application code, alongside a lightweight runtime manager executing on the host processor. 
The static compiler handles DFG (dataflow graph) generation, data partitioning, and data allocation. 
Concurrently, the runtime manager processes the data partitions, generating \textit{static AMs} that include the intermediate, final destinations and their designated locations for preloading into the \textit{AM Queues} within the PEs.
The dynamic routing is inherently done by \textit{Nexus Machine}'s architecture.
%The \textit{Nexus Machine}'s compiler produces a binary representation that encompasses the application loop kernel, data distribution across memories, and the generation of static AMs containing input operands and their precise location within the PE array.

\textbf{Static Compiler.}
Fig.~\ref{fig:compiler} illustrates the process of converting both the serial code and associated data into configurations suitable for the \textit{Nexus Machine} along with a compatible data format.

\begin{comment}
We generate the LLVM Intermediate Representation (IR) from the application's annotated C source code. 
This IR represents the low-level operations performed on data along with their dependencies.
We implement an LLVM pass to examine the LLVM IR and generate a DFG, which is translated into opcodes for the \textit{configuration memory}.
With the LLVM pass, first, backedges are identified and basic blocks are connected to establish a clear control flow. Transfer variables among nested loops are then identified, facilitating data movement across loop iterations. Subsequently, LLVM IR instructions are converted into nodes for the DFG. We then set data dependency constraints to ensure proper execution order and data integrity. Next, we remove redundant and dead DFG nodes to optimize the graph structure. Finally, the remaining DFG nodes are sorted by As Soon As Possible (ASAP) order to prioritize their execution. 
\end{comment}
We generate the LLVM Intermediate Representation (IR) from the application's annotated C source code. 
This IR captures the low-level data operations and their dependencies. 
We then apply an LLVM pass to analyze the IR and produce a Data Flow Graph (DFG), which is converted into opcodes for the \textit{configuration memory}.
The LLVM pass begins by identifying backedges and connecting basic blocks to define a clear control flow. 
It then converts LLVM IR instructions into nodes in the DFG. 
Data dependency constraints are set to ensure correct execution order and data integrity. 
Redundant and dead nodes are subsequently removed to optimize the graph structure. 
Finally, the remaining DFG nodes are sorted in As Soon As Possible (ASAP) order to optimize execution.
Fig.~\ref{fig:exec_model} illustrates a representative DFG for SpMV.

\textit{Problem definition for distributed data placement}:
Given a set of sparse tensors represented as $A$ and a reconfigurable architecture with $N$ homogeneous PEs, we employ a greedy partitioning strategy to divide $A$ into $N$ partitions, denoted as {$A_1$, $A_2$, $A_3$,...,$A_N$} as discussed in Section~\ref{section:data_placement}.
%Given a set of sparse tensors represented as $A$ and a CGRA with $N$ homogeneous PEs, we employ a greedy partitioning strategy to divide $A$ into $N$ partitions, denoted as {$A_1$, $A_2$, $A_3$,...,$A_N$}, ensuring each partition contains at least $nnz(A)/N$ non-zero elements.
%An exemplary illustration of the tensor partitioning for the SpMV kernel is detailed in Section ~\ref{section:data_placement}.
%Each partition $A_n$ is assigned to a distinct PE within the CGRA. 
%The primary objective is to maximize parallelism while minimizing communication overhead, which is quantified by ensuring that the computational cost $\phi(A_n)$ for each partition $A_n$ is minimal.%approximately equals a predefined constant $\Phi$.
The primary objective is to allocate each partition $A_n$ to a distint PE to maximize parallelism while minimizing communication overhead. This is achieved by minimizing the computational cost $\phi(A_n)$ for each partition $A_n$.

Considering two sets of tensors, denoted by $X$ and $Y$, which results in the output tensor $Z$, the optimization problem requires determining the optimal placement of these three distributed tensors. 
The output tensor $Z$ is computed as $Z = f(X, Y)$, where $f$ represents the function that operates on $X$ and $Y$ to generate $Z$. 
Initially, the partitions of $Z$ are sequentially placed on distinct PEs. 
Subsequently, the partitions of tensors $X$ and $Y$ are strategically placed based on the data dependencies inferred from the DFG.

To optimize the placement of partitions of tensor $X$, we iteratively evaluate the available partitions of $X$ and select the partition $X_{i'}$ containing the maximum number of elements required to compute the corresponding partition $Z_i$ according to the function $f(X, Y)$. 
Upon assigning $X_{i'}$ to PE $i$, it is removed from the set of available partitions. 
A similar procedure is followed for the partitions of tensor $Y$.
%Given a set of sparse tensors represented as $A$ and a CGRA with $N$ homogeneous PEs, the problem is to determine the optimal partitioning of $A$, denoted as {$A_1$, $A_2$, $A_3$,...,$A_N$}. This partitioning aims to maximize parallelism that satisfies $\phi(A_n) \simeq \Phi$, where $\phi(A_n)$ represents the computational cost of partition $n$ for $n \in {1, 2, ..., N}$, and $\Phi$ denotes a predefined constant.

%To accomplish our objectives, we implement a heuristic-driven data partitioning mechanism. Consider two sets of sparse tensors, denoted by $X$ and $Y$, that yield the set of sparse outputs, $Z$. Employing a straightforward load balancing approach, we evenly partition $Z$ into subsets: {$Z_1$, $Z_2$, $Z_3$, ..., $Z_N$}, ensuring uniform distribution across multiple PEs.
%We strategically distribute and position the input data $X$ and $Y$ based on the data dependencies from the Data Flow Graph (DFG). 
%Our placement approach aims to enhance parallelism by co-locating inputs that exhibit sequential dependencies with the output within the same PE. 
%This placement strategy optimizes the computational cost, quantified by the number of non-zero elements.

\textbf{Lightweight Runtime Manager.}
The \textit{Runtime Manager}, operating concurrently on the host processor, utilizes data placement information provided by the static compiler to generate a sequence of \textit{static AMs}.
These \textit{static AMs} are then loaded into the \textit{AM Queues} of individual PEs for execution.
Fig.~\ref{fig:message_format} illustrates the format of these compiler-generated \textit{static AMs}.
Each \textit{static AM} corresponds to a unique \textit{Op1} operation and is loaded onto the respective PE, aligned with its designated location.
Each \textit{static AM} contains the value of first operand, along with essential details such as the PE ID, and address for the dependent input operands and the result.
%A distinct \textit{static AM} is created for each computation on an output element, and these AMs are loaded onto the respective PEs aligned with the output's designated location.
%Each \textit{static AM} includes essential information such as the PE ID and data/register location details for every dependent input operand.

For every element in the first operand, the runtime manager generates a \textit{static AM} containing information about the operands and the result. 
This AM pairs this element, stored as \textit{Op1}, with the location of the second operand denoted by \textit{R1}, indicating the PE where it resides, and stores the local address as \textit{Op2}. 
Similarly, the result is stored at \textit{R2}, along with its local address as \textit{Result}.


\textbf{Static Compiler.}
Fig.~\ref{fig:compiler} illustrates the process of converting both the serial code and associated data into configurations suitable for the \textit{Nexus Machine} along with a compatible data format.
We generate the LLVM Intermediate Representation (IR) from the application's annotated C source code. 
This IR captures the low-level data operations and their dependencies. 
We then apply an LLVM pass to analyze the IR and produce a Data Flow Graph (DFG), which is converted into opcodes for the \textit{configuration memory}.
The LLVM pass begins by identifying backedges and connecting basic blocks to define a clear control flow. 
It then converts LLVM IR instructions into nodes in the DFG. 
Data dependency constraints are set to ensure correct execution order and data integrity. 
Redundant and dead nodes are subsequently removed to optimize the graph structure. 
Finally, the remaining DFG nodes are sorted in As Soon As Possible (ASAP) order to optimize execution.
Fig.~\ref{fig:exec_model} illustrates a representative DFG for SpMV.

\paragraph*{Problem Definition for Distributed Data Placement:}
Given a set of sparse tensors \( A \) and a reconfigurable architecture with \( N \) homogeneous PEs, the challenge is to assign tensor elements across PEs to balance load and minimize communication. Effective data placement is essential in distributed memory architectures for sparse tensor algebra, as it impacts both memory efficiency and execution performance.

A key tradeoff arises: minimizing communication enhances data locality but limits opportunities for opportunistic execution via AMs. Conversely, increased communication allows idle PEs to execute embedded AMs, potentially improving throughput.

Let a sparse tensor \( T \) be partitioned into disjoint subsets \( T_1, T_2, \ldots, T_P \), each assigned to \( \text{PE}_i \). The mapping function:
\[
f: T \rightarrow \{\text{PE}_1, \text{PE}_2, \ldots, \text{PE}_P\}
\]
is optimized to maximize locality, such that:
\[
\mathbb{P}(f(x) = \text{PE}_i \mid x \in T_i)
\]
is as high as possible.

\paragraph*{Motivation for Load Balancing:}
Achieving balanced memory usage often requires placing nonzeros remotely, leading to cross-PE accesses. This overhead is exploited by the AM paradigm in the \textit{Nexus Machine}, where idle PEs along communication paths execute AMs, increasing utilization and hiding latency.

\paragraph*{Dissimilarity-Aware Mapping Strategy}
Similar to previous works, \textit{Nexus Machine} uses a dissimilarity-aware placement scheme. Let \( L_i \subseteq \mathbb{M} \) be the memory banks accessed by row \( i \), and define dissimilarity as:
\[
d(i,j) = |L_i \Delta L_j|.
\]
The row-level mapping function:
\[
f_r: R \rightarrow \{\text{PE}_1, \ldots, \text{PE}_P\}
\]
groups rows with similar access patterns (low \( d(i,j) \)) to the same PE, while distributing dissimilar ones to avoid contention. This strategy supports efficient AM execution and scalable performance across diverse sparse workloads.


\textbf{Static Compiler.}

Fig.~\ref{fig:compiler} illustrates the transformation of annotated C code and associated data into executable configurations and compatible data formats for the \textit{Nexus Machine}. The source is first translated into LLVM Intermediate Representation (IR), capturing low-level operations and data dependencies. A custom LLVM pass processes this IR to construct a Data Flow Graph (DFG), which is then compiled into configuration memory opcodes.

The compiler identifies control flow using backedges and connects basic blocks. It maps IR instructions to DFG nodes, enforces data dependencies, eliminates redundant nodes, and schedules instructions in As Soon As Possible (ASAP) order. Fig.~\ref{fig:exec_model} shows a DFG example for SpMV.

\paragraph*{Problem Definition for Distributed Data Placement:}
Given sparse tensors \( A \) and a reconfigurable system with \( N \) PEs, the goal is to assign tensor elements to PEs to balance memory and reduce communication. Locality improves data access efficiency but reduces AM opportunities; more communication enables opportunistic execution via AMs.

Let tensor \( T \) be split into \( T_1, T_2, \ldots, T_P \), assigned via mapping:
\[
f: T \rightarrow \{PE_1, PE_2, \ldots, PE_P\},
\]
optimized to maximize:
\[
\mathbb{P}(f(x) = PE_i \mid x \in T_i).
\]

\paragraph*{Motivation for Load Balancing:}
Some remote data access is inevitable. In \textit{Nexus Machine}, such communication is exploited via AMs, where idle PEs assist with computation, improving overall throughput.

\paragraph*{Dissimilarity-Aware Mapping Strategy}
\textit{Nexus Machine} adopts a dissimilarity-driven placement. Let \( L_i \subseteq \mathbb{M} \) denote memory banks accessed by row \( i \). Define:
\[
d(i,j) = |L_i \Delta L_j|.
\]
Mapping function \( f_r: R \rightarrow \{PE_1, \ldots, PE_P\} \) co-locates similar rows (low \( d(i,j) \)) and spreads dissimilar ones, balancing memory access and enhancing AM execution scalability.



\begin{algorithm}[ht]
\caption{Dissimilarity-Aware Row Partitioning}
\begin{algorithmic}[1]
\Require CSR tensor \( T \), number of PEs \( P \), memory banks \( \mathbb{M} \)
\Ensure Mapping \( f_r: R \rightarrow \{PE_1, \ldots, PE_P\} \)
\For{each row \( r_i \) in CSR}
    \State \( L_i \gets \text{AccessedBanks}(r_i) \) \Comment{From column indices}
\EndFor
\For{each \( (r_i, r_j) \)}
    \State \( d(i,j) \gets |L_i \Delta L_j| \) \Comment{Symmetric difference}
\EndFor
\State \( \{C_1, \ldots, C_P\} \gets \text{Cluster}(R, d(i,j)) \) \Comment{Group similar rows}
\For{each cluster \( C_k \)}
    \State \( f_r(r) \gets PE_k \quad \forall r \in C_k \) \Comment{Assign to PE}
\EndFor
\State \Return \( f_r \)
\end{algorithmic}
\end{algorithm}




\begin{comment}

In distributed-memory architectures for sparse tensor algebra, memory partitioning is critical for load balancing and minimizing communication overhead. Formally, consider a sparse tensor T whose non-zero elements are partitioned into segments T1,T2,…,TPT_1, T_2, \ldots, T_PT1,T2,…,TP, each allocated to a dedicated processing element (PE). The mapping function f:T→{PE1,PE2,…,PEP}f: T \to \{PE_1, PE_2, \ldots, PE_P\}f:T→{PE1,PE2,…,PEP} is designed to maximize data locality so that, if x∈Tx \in Tx∈T is accessed during computation, it is most likely to reside on the same PE, thereby reducing expensive inter-PE memory accesses. However, to ensure a uniform distribution of non-zero elements across available memory banks, some data must inevitably be stored remotely. Although this results in occasional cross-PE accesses, the architecture exploits such interactions within the active message (AM) paradigm of the Nexus Machine by allowing idle PEs to opportunistically execute computations along the communication path, which ultimately improves overall system utilization and reduces latency.
Building on insights from state-of-the-art accelerators (e.g., ZeD and Gamma), the architecture adopts a dissimilarity-driven mapping strategy to further optimize performance. Specifically, let LiL_iLi denote the set of memory banks accessed by the non-zero entries in the i-th row of the sparse tensor. A dissimilarity score d(i,j)=∣LiΔLj∣d(i,j) = |L_i \Delta L_j|d(i,j)=∣LiΔLj∣ is defined for each pair of rows, where Δ\DeltaΔ denotes the symmetric difference. Rows with low dissimilarity scores—i.e., those with substantial overlap in their memory bank access patterns—are grouped and mapped onto a single Nexus PE, thereby reducing potential contention on individual memory banks. Conversely, rows with high dissimilarity scores are distributed across different PEs to ensure that concurrently spawned active messages do not overload the same network paths or memory banks.
 
an inherent inefficiency that is exploited as a benefit by the AM paradigm of Nexus Machine
\end{comment}
